Subpacketization-Rate Trade-off in Multi-Antenna Coded Caching

Coded caching can be applied in wireless multi-antenna communications by multicast beamforming coded data chunks to carefully selected user groups and using the existing file fragments in user caches to decode the desired files at each user. However, the number of packets a file should be split into, known as subpacketization, grows exponentially with the network size. We provide a new scheme, which enables the level of subpacketization to be selected freely among a set of predefined values depending on basic network parameters such as antenna and user count. A simple efficiency index is also proposed as a performance indicator at various subpacketization levels. The numerical examples demonstrate that larger subpacketization generally results in better efficiency index and higher symmetric rate, while smaller subpacketization incurs significant loss in the achievable rate. This enables more efficient caching schemes, tailored to the available computational and power resources.

==> SystemModelDraft.tex <==
Assume each file is divided into $P$ equal-sized subpackets. In order to better represent the cache placement scheme we define a binary placement matrix $\mathbf{Q}$ of size $P \times S$. For every $p \in [P]$ and $s \in [S]$, if $q_{p,s} = 1$ then for any file $Z$ in the file library we store $Z_p$ at the cache memory of user $s$, where $Z_p$ is the $p$-th subpacket of $Z$. For example if $S = 4$ then
\begin{equation}
\label{eq:Q_mat_4_2_T1}
    \mathbf{Q} = 
    \begin{bmatrix}
    1 & 1 & 0 & 0 \\
    0 & 1 & 1 & 0 \\
    0 & 0 & 1 & 1 \\
    1 & 0 & 0 & 1
    \end{bmatrix}
\end{equation}
represents a cache placement for which each file is divided into 4 subpackets and $\{ A_1, A_4, B_1, B_4, ... \}$ are stored at the cache memory of user 1, $\{ A_1, A_2, B_1, B_2, ... \}$ are stored at the cache memory of user 2, and so on. We say $\mathbf{Q}$ is a valid placement matrix, if for each row and column of $\mathbf{Q}$ sum of the elements is $t$ and $\frac{Pt}{S}$, respectively. It can be easily checked that if $\mathbf{Q}$ is valid the cache size constraint of $MF$ bits for all the users is satisfied. Furthermore, the original cache placement of [...] is equivalent to any valid placement matrix with $P = \binom{S}{t}$, while the cache placement represented in [...] is equivalent to any valid placement matrix with $P = \frac{t}{L}$.

At the beginning of the delivery phase the users reveal their requested files. Assume the file requested by user $s$ is represented by $Z^{\{s\}}$. If $q_{p,s} = 0$, $Z^{\{s\}}_p$ should be delivered to user $s$ during delivery phase. Now consider row $p$ of the placement matrix $\mathbf{Q}$. According to the validity conditions we know this row has exactly $t$ elements of value 1, which means $Z^{\{s\}}_p$ is stored at the cache memories of $t$ users in the network; and these users can delete $Z^{\{s\}}_p$ from their received codewords. Although as we have $L$ antennas, we can zero-force the transmission for $L-1$ other users. Assume the zero-forcing transmission vector is denoted by $\mathbf{u}_{p,s}$. So transmitting $Z^{\{s\}}_p \mathbf{u}_{p,s}$, enables user $s$ to receive $Z^{\{s\}}_p$ while causing no interference at other users. This property enables $Z^{\{s\}}_p$ to be XOR-ed with other file parts which are going to be transmitted with the same transmission vector. For example, for the placement matrix $\mathbf{Q}$ of \eqref{eq:Q_mat_4_2_T1} it can be easily verified that $\mathbf{u}_{1,3} = \mathbf{u}_{2,1} = \mathbf{h}_4^{\perp}$; and hence by transmitting $(Z^{\{3\}}_2 \oplus Z^{\{2\}}_1) \mathbf{h}_4^{\perp}$ enables users 1 and 2 to decode $Z^{\{2\}}_1$ and $Z^{\{3\}}_2$ respectively, while causing no interference at users 3 and 4. So the transmitter has to first XOR all terms with the same transmission vectors, and then transmit all the resulting terms with appropriate powers; and all users will be able to decode all their requested data.

Still lacks good data flow and important parts:
\begin{enumerate}
    \item Start from the system model. It should be described first.
    \item Better explanation of what's happening is required. Maybe the example position should be changed.
    \item Better representation for transmission matrices is needed.
    \item Better codeword creation and transmission vector creation explanation is needed.
    \item This how to move to the efficiency index.
    \item Think how to integrate the results with the multi-server scheme. Maybe this is the most difficult part.
    \item Should we provide examples showing equivalency with Petros and multi-server schemes?
\end{enumerate}

Maybe the flow should be changed:
\begin{enumerate}
    \item A short description of the multi-server scheme and stating that we are just considering subsets of size $S$. I should explain that the placement in multi-server scheme is in fact consisting of two phases, and I'm just considering the first phase.
    \item Then is the right time to introduce the placement matrix. The current representation is not bad for that.
    \item Then I should present codeword and transmission vector creation process. This needs further focus. How codewords are created, how transmission vector is created, and what is received at each user. Maybe I should not go into details that why interference is cancelled - instead provide the formula only and explain everything through examples. It would be nice if I can get feedback for that from someone professional.
    \item I think here the chapter should be finished. The definition of efficiency index and the reasoning behind it should be left for the next chapter.
\end{enumerate}

----------------------------------
